Learning Neural Ranking Models Online from Implicit User Feedback

Existing online learning to rank (OL2R) solutions are limited to linear models, which are incompetent to capture possible non-linear relations between queries and documents. In this work, to unleash the power of representation learning in OL2R, we propose to directly learn a neural ranking model from users' implicit feedback (e.g., clicks) collected on the fly. We focus on RankNet and LambdaRank, due to their great empirical success and wide adoption in offline settings, and control the notorious explore-exploit trade-off based on the convergence analysis of neural networks using neural tangent kernel. Specifically, in each round of result serving, exploration is only performed on document pairs where the predicted rank order between the two documents is uncertain; otherwise, the ranker's predicted order will be followed in result ranking. We prove that under standard assumptions our OL2R solution achieves a gap-dependent upper regret bound of $O(\log^2(T))$, in which the regret is defined on the total number of mis-ordered pairs over $T$ rounds. Comparisons against an extensive set of state-of-the-art OL2R baselines on two public learning to rank benchmark datasets demonstrate the effectiveness of the proposed solution.

==> arxiv_problem.tex <==
\section{Problem Formulation}
In this section, we provide a brief overview about the general problem setting in OL2R, especially about its key challenges, and the notion of fairness in ranking employed in this paper.

\subsection{Online Learning to Rank}

In OL2R, at round $t \in [T]$, the ranker receives a query $q_t$ and its associated $L_t$ candidate documents\footnote{We will use ``document'' and ``item'' interchangeably in this paper to denote the instances to be ranked under a query.} represented by a set of $d$-dimensional query-document feature vectors: $\mathcal{X}_t = \{\xb_1^t, ..., \xb_{L_t}^t\}$ where $\xb^t_i \in \RR^d$. 
The ranking $\pi_t = \big(\pi_t(1), ..., \pi_t(L_t)\big) \in \Pi([L_t])$ is generated by the ranker based on its knowledge so far and its exploration strategy, where $\Pi([L_t])$ represents the set of all permutations of $L_t$ documents and $\pi_t(i)$ is the rank position of document $i$. The user examines the returned ranked list and provides his/her feedback, i.e., clicks $C_t = \{c_1^t, c_2^t, ..., c_{L_t}^t\}$, where $c_i^t = 1$ if the user clicked on document $i$ at round $t$; otherwise $c_i^t = 0$. According to the collected implicit feedback, the ranker updates itself for improved ranking in the next round.

As the ranker learns from user feedback while serving, cumulative regret is an important metric for evaluating an OL2R solution. Usually regret is defined as the cumulative expected difference between the utility of the presented ranked list $\pi_t$ and that of the ideal one $\pi_t^*$ over a finite time horizon $T$, i.e., 
\begin{equation}
\label{eq_regret_def}
    R_T = \mathbb{E}\left[\sum\nolimits_{t=1}^T r_t\right] = \mathbb{E} \left[\sum\nolimits_{t=1}^T f(\pi_t^*) - f(\pi_t)\right],
\end{equation}
where $f(\cdot)$ represents a chosen utility function. $f(\cdot)$ can be set as the number of clicks \citep{kveton2015cascading,lattimore2018toprank} or the number of correctly ordered pairs of documents \citep{jia2021pairrank}, based on the application context of OL2R. 

We have to emphasize that OL2R is \emph{\textbf{not}} literally just learning a ranking model online, such as using online gradient descent over a parametric model. The key challenge is the ranker only learns from the feedback collected in its presented rankings -- the so-called bandit feedback \citep{lattimore2020bandit}. For the results not presented to the users (i.e., presentation bias) or those presented at lower positions (i.e., position bias), the ranker has little knowledge about their relevance. As a result, the ranker has to repeatedly present the currently underestimated results on top for more feedback, which however contradicts its need to present the currently best ranking to reduce instantaneous regret. This is the well-known explore-exploit dilemma in OL2R. And the extremely large ranking space, i.e., exponentially sized possible rankings, further amplifies the difficulty in OL2R.
%The challenges in OL2R are two-fold: in addition to the well-known explore-exploit trade-off in all online learning problems with bandit feedback,  
Efficient exploration is thus needed to shrink the search space so as to quickly find satisfying result rankings to reduce regret. As discussed in Section \ref{sec_related}, various exploration strategies have been proposed in literature, with their own advantages and limitations. Our work in this paper is not to develop yet another OL2R solution, but to provide a general framework that ensures ranking fairness in a family of existing OL2R solutions. 

\subsection{Fairness in OL2R}
It is asserted by the probability ranking principle that user-side utility reaches its optimal when the documents are ranked by the expected values of their estimated relevance (merit) to the user \citep{robertson1977probability}. However, it unfortunately ignores the differential treatment that content providers would receive from the document side in such rankings.  
The key resource that a ranking system allocates among the documents is exposure \citep{singh2018fairness}, which influences the probability that the documents to be examined by the users and consequentially the social and/or economic benefit the content provider will receive. 
Without loss of generality, in this work, we assume all ranking candidates among all queries over time belong to two groups ($G_A$ and $G_B$). We define the instantaneous unfairness resulted in a particular ranked list as the difference between the exposure received by group $G_A$ and group $G_B$ from the presented ranking,
\begin{align*}
    UF(G_A, G_B, \beta) = Exposure(G_A) - \beta Exposure(G_B),
\end{align*}
where $\beta$ is an unfairness coefficient that controls the relative exposure that group $G_A$ and $G_B$ should receive. $\beta$ is an hyper-parameter chosen by the system designer to weigh the discrepancy in exposure between the two groups based on the need of specific applications. The definition of exposure is also application-specific: it can be quantified as the examination probability \citep{morik2020controlling} or the clicks/dwelling time received by the ranked documents. In this work, we adopt the classical choice of examination probability to simplify our discussion, but our solution can be generalized to other definitions with specific instrument to measure/infer the corresponding exposure.

To capture the difference of the cumulative treatment received during the course of OL2R up to time $t$, we consider a ranking system fair, if for any $t\in[T]$, we have
\begin{align}
\label{eqn:unfairness}
    UF_t = \left|\sum\nolimits_{s=1}^t\Big(Exposure_s(G_A) - \beta Exposure_s(G_B)\Big)\right|\le\epsilon,
\end{align}
where $\epsilon>0$ is a threshold chosen by the system designer to satisfy task-specific requirement of fairness. 

Our definition of unfairness is general to cover most of the existing exposure-based ranking fairness metrics. First, for demographic parity constraint proposed in \citep{singh2018fairness} which enforces that the average exposure of groups to be equal, $\beta$ can be set as the expected ratio of the group sizes between $G_A$ and $G_B$; while for fairness concerning the disparate treatment \citep{singh2018fairness, morik2020controlling}, of which the exposure received by each group should be proportional to their relevance or merit, $\beta$ can be set as the ratio of expected utility between groups. Besides, our unfairness definition is not limited to only two groups. Different pairs of groups can have different $\beta$ to control the relative exposure as long as the $\beta$s satisfy the transitivity constraint.

